Design-Time Quantification of Integrity in Cyber-Physical-Systems

In a software system it is possible to quantify the amount of information that is leaked or corrupted by analysing the flows of information present in the source code. In a cyber-physical system, information flows are not only present at the digital level, but also at a physical level, and to and fro the two levels. In this work, we provide a methodology to formally analyse a Cyber-Physical System composite model (combining physics and control) using an information flow-theoretic approach. We use this approach to quantify the level of vulnerability of a system with respect to attackers with different capabilities. We illustrate our approach by means of a water distribution case study.

==> sections/CPS-IFT_old.tex <==
%\subsection{Attacker model}
%These physical variables are represented in our CPS model by the output of the process $y$, which is a vector of analogue observations of the physical variables. Ultimately, our notion of security will depend on the vector $y$. %The attacker will launch both physical and cyber attacks depending on her capabilities. %Clearly, if the attacker is too powerful, then she will succeed.
%
%The $k$-cycle execution is characterised by the semantics function
%\begin{align}
%\TheSystem^k&= \TheSystem \circ \TheSystem^{k-1}.
%\end{align}
%where $\circ$ is function composition.
%
%%Although CPS are meant to run indefinitely, we characterise finite executions to better characterise noninterference our model of CPSs. 
%The single-cycle semantics updates the state $cps_{k}=(y_{k}, u_{k},\hat{u}_{k},\hat{y}_{k})$ to the state $cps_{k+1}=(y_{k+1}, u_{k+1},\hat{u}_{k+1}, \hat{y}_{k+1})$. Formally, 
%\begin{align}
%cps_{k+1}&=\TheBehaviourOf{(y_{k}, u_{k},\hat{u}_{k},\hat{y}_{k})}\\
%&=\left(\TheBehaviourOf{\hat{y}_{k}}_{AD},\TheBehaviourOf{y_{k}}_{IO}, \TheBehaviourOf{u_{k}}_{DA},  \TheBehaviourOf{\hat{u}_{k}}_{\Phi}\right).%\\
%%&=(y_{k+1}, u_{k+1},\hat{u}_{k+1}, \hat{y}_{k+1}).
%%&=\TheBehaviourOf{cps_{k}}.
%\end{align}
%Clearly, if the attacker controls all the sensor data, i.e., the vector $y$, then she has full control over the vector of control signals $u$, modulo the semantics $\TheBehaviourOf{}_{IO}$.
%To formally define an attacker, we select a subset of components that we assume the attacker controls. 
% %Let us call this attacker an \emph{IF-attacker}. 
%Let $S=\set{s_1, \ldots, s_n}$ be the set of sensors, and let $y_s$ be the component of the vector $y$ of sensor data that corresponds to sensor $s$. 
%We say that an attacker controls sensor $s$ if she can replace $y_s(k)$ with an arbitrary value $\bar{y}_s(k)$, for all $k$. Formally, for all $k$, 
%\begin{align}
%\bar{y}(k) := [\bar{y}_s(k)/y_s(k)]y(k),
%\end{align} 
%where $[\bar{y}_s(k)/y_s(k)]y(k)$ reads ``substitute $y_s(k)$ by $\bar{y}_s(k)$ in $y(k)$.'' If the attacker does not control a sensor $s'$, then $\bar{y}_{s'}(k)={y}_{s'}(k)$, for all $k$.
%
%Similarly, let $A=\set{a_1, \ldots, a_m}$ be the set of actuators, and let ${u}_a$ be the component of the vector ${u}$ of control actions that corresponds to actuator $a$. We say that an attacker controls actuator $a$ if she can replace $\hat{u}_a(k)$ with an arbitrary control action $\bar{{u}}_a(k)$, for all $k$. Formally, for all $k$
%\begin{align}
%\bar{{u}}(k) :=[\bar{\hat{u}}_a(k)/u_a(k)] u(k).
%\end{align}
%Thus, we represent an {IF-attacker} with a set $\alpha \subseteq A\cup S$.
%%Finally, let $\hat{u}_a$ be the component of the vector $\hat{u}$ of physical actions that corresponds to the interface $p$. 
%%
%%We say that an attacker controls a physical action $p$ if she can replace $\hat{u}_a(k)$ with an arbitrary effect $\bar{\hat{u}}_a(k)$, for all $k$. Formally, for all $k$, 
%%\begin{align}
%%\bar{u}(k) := u(k)[\bar{u}_a(k)/u_a(k)],
%%\end{align}.
%%We represent an \emph{IF-attacker} by a subset of $A\cup S$.

%The IF-attacker model is compatible with the notion of attackers discussed in \S \ref{sec:CT}, though an IF-attacker does not mind being detected as long as she accomplishes her goal. 
%Henceforth, we will consider possibly corrupted sensor measurements $\bar{y}$ and control actions $\bar{u}$. Thus, following Definition \ref{def:SingleCycleSemantics}, the single-cycle semantics updates the state $(\bar{y}(k), \bar{u}(k),\hat{u}(k),\hat{y}(k))$ to the state $(\bar{y}(k+1), \bar{u}(k+1),\hat{u}(k+1), \hat{y}(k+1))$. Formally, $\TheBehaviourOf{(\bar{y}(k), \bar{u}(k),\hat{u}(k),\hat{y}(k))}$ is equal to 
%\begin{align}
%&\left(\TheBehaviourOf{\hat{y}(k)}_{AD},\TheBehaviourOf{\bar{y}(k)}_{IO}, \TheBehaviourOf{\bar{u}(k)}_{DA},  \TheBehaviourOf{\hat{u}(k)}_{\Phi}\right)
%%&=(y(k+1), u(k+1),\hat{u}(k+1), \hat{y}(k+1)).
%%&=\TheBehaviourOf{cps(k)}.
%\end{align}
%We say that the system is vulnerable if the attacker, by only using her given capabilities, can control the critical physical component(s) (which are determined by experts).

% We remark that we do not allow IF-attackers to directly control physical actions. For example, if the attacker uses a signal jammer, she is exerting a physical action that affects the state of the physical part of the receiver. This restriction is sensible at design level, because design focuses on the physical process and its model, ultimately relying on physical security to protect physical components from the attacker once the CPS is implemented. Thus, we would consider attacks directly on the physics of the implemented CPS to be \emph{side-channel attacks} on the integrity of the CPS, which are outside the scope of this work. 

%We remark that an IF-attacker could have capabilities both in the digital and in the physical worlds. We do abstract from the means an IF-attacker uses to corrupt $y$ and/or $\hat{u}$.
% and she might not be restricted to only changing sensor measurements or control signals.  

%We assume that the attacker has full control over her capabilities; e.g., if the attacker controls a water level sensor, then she can send any water level measurement she desires to the PLCs at any point she thinks is convenient. 

%
%Let $cps_{[1]}=(\bar{y}_{[1]},\bar{u}_{[1]},\hat{u}_{[1]}, \hat{y}_{[1]})$ and $cps_{[2]}=(\bar{y}_{[2]},\bar{u}_{[2]},\hat{u}_{[2]}, \hat{y}_{[2]})$ be abstract states of the CPS. We say that $cps_{[1]} =_{\High} cps_{[2]}$ iff for all components $c$ of the CPS, 
%\begin{align}
%&\begin{cases}
%{(\bar{y}_{[1]})_c}={(\bar{y}_{[2]})_c}, & \text{if $c\not\in \alpha$}\\
%True, & \text{otherwise}\\
%\end{cases}& \text{ and }\quad & 
%\begin{cases}
%(\bar{u}_{[1]})_c=(\bar{u}_{[2]})_c, & \text{if $c\not \in \alpha$}\\
%True, & \text{otherwise}\\
%\end{cases}\\
%& \text{ and }\hat{u}_{[1]}=\hat{u}_{[2]}& \text{ and }\quad & \hat{y}_{[1]}=\hat{y}_{[2]}.
%\end{align}
%
%and we say that the behaviours 
%$\TheBehaviourOf{cps_{[1]}}$ and $\TheBehaviourOf{cps_2}$ are \emph{$\hat{y}$-equivalent}, denoted $\TheBehaviourOf{cps_{[1]}}\approx_{\hat{y}} \TheBehaviourOf{cps_{[2]}}$ iff $\TheBehaviourOf{\hat{u}_{[1]}}_{\Phi}= \TheBehaviourOf{\hat{u}_{[2]}}_{\Phi}$. 
%
%Finally, we say that the CPS satisfies noninterference against the IF-attacker $\alpha$ if and only if, for all abstract states $cps_{[1]}=(\bar{y}_{[1]},\bar{u}_{[1]},\hat{u}_{[1]}, \hat{y}_{[1]})$ and $cps_{[2]}=(\bar{y}_{[2]},\bar{u}_{[2]},\hat{u}_{[2]}, \hat{y}_{[2]})$ we have
%\begin{align}
%\label{eq:NoninterferenceCPS}
%cps_{[1]} =_{\High} cps_{[2]} \Rightarrow \TheBehaviourOf{cps_{[1]}} \approx_{\hat{y}} \TheBehaviourOf{cps_{[2]}}.
%\end{align}
%, because an IF-attacker may alter eventually c signal of a 

%Following the non-interference framework, we consider analog observations to be $\High$ outputs, and we consider the inputs by the attacker to be $\Low$ inputs. 
%We now work towards providing an answer to two interesting and relevant questions: 1) given an IF-attacker, how do we verify that the system is secure? and 2) given a vulnerable system, how can we change the logic of the programs so that we protect the system against the attacker?
%system and a target physical component, which other components are the most profitable for attackers to control in order to interfere with the targetted component?

%\[((\bar{y},\bar{y}^*),\bar{u},(\hat{u},\hat{u}^*), \hat{y})\]
%$\TheBehaviourOf{(\bar{y}(k), \bar{u}(k),\hat{u}(k),\hat{y}(k))}$ is now equal to 
%\begin{align*}
%&\left(\TheBehaviourOf{\hat{y}(k)}_{AD},\TheBehaviourOf{\bar{y}(k), \bar{y}^*(k)}_{IO}, \TheBehaviourOf{\bar{u}(k)}_{DA},  \TheBehaviourOf{\hat{u}(k),\hat{u}^*(k)}_{\Phi}\right).
%%&=(y(k+1), u(k+1),\hat{u}(k+1), \hat{y}(k+1)).
%%&=\TheBehaviourOf{cps(k)}.
%\end{align*}
%In other words, 
%the analysis remains essentially the same, with the difference that the semantics of the program now depends on both sensor measurements (i.e., $\bar{y}$) and digital messages sent by the other CPS (i.e., $\bar{y}^*$), and the semantics of the physics now depends on both physical actions carried out by the actuators (i.e., $\hat{u}$) and physical effects due to physical laws (i.e., $\hat{u}^*$).

%We remark that an attacker cannot act as MiTM in the classical sense between the two physics, because that would require the attacker to be able to change the laws of physics, which is an unreasonable assumption. Nevertheless, an IF-attacker can exploit the existence of those channels opened by the laws of physics in order to propagate her interference. 
%There are two continuous variables, denoted by $l(t)$ (the water level) and $\delta(t)$ (time elapsed since last signal was sent by the controller).There are also two discrete variables, denoted by $P(t)$ (the status of the pump, taking values in $\set{on,off}$) and $S(t)$ (the nature of the signal sent by the monitor, also taking values in $\set{on,off}$). The dynamics, as given in \cite{TheAlgotihmicAnalysisOfHybridSystems,ModelingAndControlOfHybridDynamicalSystems}, is as follows. The water level rises one unit per econd when the pump is on and falls two units per second when the pump is off. When the water level rises to 10 units, the monitor sends a switch-off signal, which after a delay of two secons results in the pump turning off. 

==> sections/IFT-Extra.tex <==
%!TEX root = ../EGRM-ESORICS-LNCS.tex
\subsection{Biba Integrity}
The Biba model consists of a set $\TheSetOfSubjects$ of subjects, set $\TheSetOfObjects$ of objects, and a set $\TheSetOfIntegrityLevels$ of integrity levels ordered by the relation $\leq \subseteq \TheSetOfIntegrityLevels\times \TheSetOfIntegrityLevels$. The function $\Lvl\colon \TheSetOfSubjects \cup \TheSetOfObjects \rightarrow \TheSetOfIntegrityLevels$ returns the integrity level of an object or a subject. The Biba model defines rules for $\TheSubject,\TheSubject_1,\TheSubject_2\in \TheSetOfSubjects$ and $\TheObject\in \TheSetOfObjects$ as follows.
\begin{enumerate}
\item $\TheSubject$ can read $\TheObject$ if and only if $\Lvl(\TheSubject) \leq \Lvl(\TheObject)$.
\item $\TheSubject$ can write $\TheObject$ if and only if $\Lvl(\TheObject) \leq \Lvl(\TheSubject)$.
\item $\TheSubject_1$ can execute $\TheSubject_2$ if and only if $\Lvl(\TheSubject_2) \leq \Lvl(\TheSubject_1)$.
\end{enumerate}
%Rule 1 allows flows of information from higher security levels, and Rule 2 allows flows of information to lower security levels. If we focus on information flows that can change the state of an object (Rule 2), to enforce integrity, we want to restrict ``write'' flows from low security levels to high security levels. 
The {noninterference framework} captures these three rules under one unified definition.

==> sections/OptionalContent.tex <==

\subsection{Conclusion}
We can systematically determine the dependencies among variables in a program by constructing its data-flow diagram, and we can systematically quantify how much information flows from one variable to another using a language-based approach. For our example CPS, while the dependency between $\hat{y}_l$ and $\hat{y}_h$ characterised by Equation \eqref{eq:HydrostaticPressure}, there is no equation that models the dependency between the valves. and it is also not evident how to systematically quantify this flow. 
\todo[inline]{Physical dependencies cannot be avoided, but they can be tricked. Does it make a difference to rely on states of other valves? }
\todo[inline]{How do we use QIF to determine dependencies?}
\todo[inline]{Do the QIF dependencies approach the physics of the system? or are we missing something?}
\todo[inline]{What are the QIF tools that we can use? Can we transform equations to code and then analyse them? the model from control theory is the equations!}
\todo[inline]{Can we use QIF to feed control theory to provide policies for enforcers? This would connect with McMillin's compensating pairs}


\begin{itemize}
\item We could think of modelling the control system as a blackbox with two input channels and two output channels.
\end{itemize}

%we are interested in exploring how much influence an attacker could have over a CPS. 

\begin{figure}[h]
\centering
\includegraphics[scale=0.5]{rsc/fig/simei/IFModel}
\caption{Simple water tank. We denote valves by $\bowtie$ and sensors by $\otimes$. The level sensor measures the water level, and the pressure sensor measures the pressure at the bottom of the tank.}
\end{figure}
\begin{figure}[h]
\centering
\includegraphics[scale=0.5]{rsc/fig/simei/IFlows}
\caption{Contamination measures the influence of attackers on the CPS, and suppression measures how much trusted information an attacker can prevent from flowing. Unimportant flows appear dotted.}
\end{figure}
\todo[inline]{Are the dotted flows still uninteresting? Yeah.}

\begin{table}
 \centering
  \caption{Qualitative Analysis of CPS attacker models.}
\begin{tabular}{ |cccc|ccc| } 
 \hline
\rotatebox[origin=c]{65}{Program}& \rotatebox[origin=c]{65}{Channel}&  \rotatebox[origin=c]{65}{Validity} &  \rotatebox[origin=c]{65}{Plausibility} & \rotatebox[origin=c]{65}{Contamination} &\rotatebox[origin=c]{65}{\begin{tabular}{@{}c@{}} Channel  \\ Suppression \end{tabular}}&\rotatebox[origin=c]{65}{\begin{tabular}{@{}c@{}} Program  \\ Suppression \end{tabular}}\\ 
 \hline
 $\bullet$ & $-$ & $-$ & $-$ & $\bullet$ & $\bullet$ & $\bullet$ \\ 
 \hline
  $-$ & $\bullet$ & $-$ & $-$ & $\bullet$ & $\bullet$ & $-$ \\ 
% \hline
%   $-$ & $-$ & $\bullet$ & $\bullet$ & $\bullet$ & $-$ \\ 
 \hline
    $-$ & $-$ & $\bullet$ & $-$ & $\bullet$ & $-$ & $-$\\ 
 \hline
   $-$ & $-$ & $-$ & $\bullet$ & $\bullet$ & $-$ & $-$\\ 
\hline
 \end{tabular}
 \label{tab:QualitativeAttackers}
\end{table}


\todo[inline]{Create a section of qualitative analysis and provide this definition. Do not put it here mixed with what clarkson and schneider wrote.}


==> sections/QuantificationOfIntegrity.tex <==
%!TEX root = ../EGRM-ESORICS-LNCS.tex
\subsection{Information Flow Analysis for Integrity}
%Noninterference gives us a \emph{qualitative} notion of information flows; more precisely, noninterference determines whether there is a flow from a security level to another that violates the security policy. 
Clarkson and Schneider \cite{QuantitativeIntegrity} define \emph{corruption} to be the damage to integrity that an attacker can cause to the system. They point out that quantification of {corruption} has received little to no attention when compared to quantification of information leakage, which has been researched for over two decades. This may be because confidentiality is regarded as more important than integrity in the commercial context, and integrity is handled on a qualitative basis. Nevertheless, Clarkson and Schneider state that quantitative requirements are valuable for privacy protection, \emph{e.g.}, if we contaminate information on purpose to enhance privacy. They use two formal definitions of integrity to quantify corruption: one based on \emph{taint analysis}, and one based on the notion of \emph{program correctness}. 

\emph{Contamination} is a generalisation of taint analysis, which tracks information flows from untrusted inputs to outputs that are supposed to be trusted. Let $t_{in}$, $u_{in}$ and $t_{out}$ denote trusted input, untrusted input and trusted output, respectively. The existence of flows from $u_{in}$ to $t_{out}$ results in {contamination} of the trusted outputs (see Figure \ref{fig:Contamination}). Integrity requires that trusted outputs must not be influenced by untrusted information, so contamination violates integrity. Contamination is the dual to information leakage under the Biba duality \cite{BibaIntegrity} between integrity and confidentiality.

The quantification of contamination yields a measure of how much an untrusted input interferes with the trusted output, and it is dual to quantification of information leaks, a technique for the analysis of covert channels \cite{QuantifyingInformationFlow,QIF}. Let $T_{in}$, $U_{in}$ and $U_{out}$ respectively denote the probability distributions on $t_{in}$, $u_{in}$ and $t_{out}$. For single events, the \emph{mutual information between $u_{in}$ and $t_{out}$}, denoted  $I(u_{in},t_{out})$, characterises the quantity of information that $t_{out}$ conveys about $u_{in}$. The mutual information between untrusted input $u_{in}$ and trusted output $t_{out}$ given the occurrence of the trusted input $t_{in}$ is $I(u_{in},t_{out}|t_{in})$, and it measures contamination of trusted outputs by untrusted inputs in a single execution. Clarkson and Schneider also present a quantification for contamination in sequences of executions where the attacker fixes an untrusted input value $u_{in}$ before the first execution, and the user refines her knowledge about $u_{in}$ at each execution after observing the $j^{th}$ trusted output $t^j_{out}$. We omit such discussion because, for CPSs, the attacker can change $u_{in}$ before each execution; thus, we study multiple single executions instead of one sequence of  executions. %Let $U_j$ be a random variable that represents the user's accumulated knowledge in execution $j$ about $u_{in}$; the distribution of $U_{j+1}$ is defined in terms of the distribution of $U_{j}$ by $\mathtt{Pr}(U_{j+1}=u_{in}) = \mathtt{Pr}(U_{j}=u_{in}| t^{j}_{out}, t^{j}_{in})$. The total contamination in a sequence of executions is $\sum_j I(u_{in}^j, t^j_{out}|t^j_{in})$, where $u_{in}^j$ is the untrusted input event in execution $j$, and mutual information is calculated according to the distribution of the user's accumulated knowledge $U_j$ about the untrusted input event in execution $j$ 

\begin{figure}[h]
\centering
\includegraphics[scale=0.5]{rsc/fig/simei/Contamination}
\caption{Model of contamination \cite{QuantitativeIntegrity}. Untrusted inputs are introduced by the attacker.}
\label{fig:Contamination}
\end{figure}

\emph{Suppression} is the other measure for corruption, and it derives from program correctness. In a setting where we have two agents, a \emph{sender} and a \emph{receiver}, if the specification requires the system to produce an output $o$ for a given input, and the implementation instead produces an output $o'$ such that $o'$ does not convey all the information about $o$, then \emph{program suppression} has occurred.   Figure \ref{fig:ProgramSuppression} shows a model of program suppression. Integrity requires that implementation outputs must not omit information about correct outputs (with respect to the specification), so program suppression violates integrity. The quantification of program corruption yields a measure of how much information is lost when the program produces the output $o'$ instead of $o$. There does not seem to be a Biba dual to suppression for confidentiality.

\begin{figure}[h]
\centering
\includegraphics[scale=0.5]{rsc/fig/simei/ProgramSuppression}
\caption{Program suppression model \cite{QuantitativeIntegrity} where implementation outputs are not correct.}
\label{fig:ProgramSuppression}
\end{figure}

\emph{Channel suppression} is an instantiation of program corruption where the program implements a communication channel. The quantification of channel suppression measures the amount of information a receiver fails to learn about trusted inputs by observing trusted outputs. A model of channel suppression appears in Figure \ref{fig:ChannelSuppression}. 

\begin{figure}[h]
\centering
\includegraphics[scale=0.5]{rsc/fig/simei/ChannelSuppression}
\caption{Channel suppression model \cite{QuantitativeIntegrity}.}
\label{fig:ChannelSuppression}
\end{figure}
%\todo[inline]{@Martin: I'm still missing the measure for suppression. It is similar to that of contamination, do you think we should still add it? If yes, then I'll add it.}
%In this work, we address the quantification of contamination and suppression at an abstract level. We invite the interested reader to check \cite{QuantitativeIntegrity} for the precise formulation of quantification of these two corruption measures. Instead, we discuss the potential applications of the quantification of integrity framework for CPS, and we use formulas that are closer to the physics of the system in the examples.
%\todo[inline]{If you have more time, provide more context on the story of QIF for integrity, mentioning noninterference, a bit of story that highlights that there has been a lot of research in quantification of confidentiality, but little in quantification of integrity}



==> sections/abstract.tex <==
%!TEX root = ../EGRM-ESORICS-LNCS.tex
\begin{abstract}
In a software system it is possible to quantify the amount of information that 
is leaked or corrupted by analysing the flows of information present in the 
source code. In a cyber-physical system, information flows are not only present 
at the digital level, but also at a physical level, and to and fro the two 
levels. %Motivated by an interest in quantifying the tolerance of 
%cyber-physical system to attacks on integrity, we challenge the applicability 
%of information-flow theory to cyber-physical systems security. 
In this work, we provide a methodology for coupling physical models from 
control theory with a language-based approach to formally analyse a 
Cyber-Physical System composite model using an information flow-theoretic 
approach. We use this approach to determine whether a system is 
vulnerable to attackers with different capabilities. We illustrate our approach 
by means of a water distribution case study. 
%\todo[inline]{Adapt abstract so that we ``challenge less'' and ``illustrate more''.}
\end{abstract}
